Examples and Results from a BSc-level Course on Domain Specific Languages of Mathematics

At the workshop on Trends in Functional Programming in Education (TFPIE) in 2015 Ionescu and Jansson presented the approach underlying the "Domain Specific Languages of Mathematics" (DSLsofMath) course even before the first course instance. We were then encouraged to come back to present our experience and the student results. Now, three years later, we have seen three groups of learners attend the course, and the first two groups have also continued on to take challenging courses in the subsequent year. In this paper we present three examples from the course material to set the scene, and we present an evaluation of the student results showing improvements in the pass rates and grades in later courses.

==> eptcsdata.tex <==
\providecommand{\firstpage}{79}
\providecommand{\publicationstatus}{P. Achten, H. Miller (Eds.): \\
Trends in Functional Programming in Education 2018 (TFPIE'18)\\
EPTCS 295, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.295.6}{10.4204/EPTCS.295.6}}

